Lumina-Video: Efficient and Flexible Video Generation with Multi-scale Next-DiT

Recent advancements have established Diffusion Transformers (DiTs) as a dominant framework in generative modeling. Building on this success, Lumina-Next achieves exceptional performance in the generation of photorealistic images with Next-DiT. However, its potential for video generation remains largely untapped, with significant challenges in modeling the spatiotemporal complexity inherent to video data. To address this, we introduce Lumina-Video, a framework that leverages the strengths of Next-DiT while introducing tailored solutions for video synthesis. Lumina-Video incorporates a Multi-scale Next-DiT architecture, which jointly learns multiple patchifications to enhance both efficiency and flexibility. By incorporating the motion score as an explicit condition, Lumina-Video also enables direct control of generated videos' dynamic degree. Combined with a progressive training scheme with increasingly higher resolution and FPS, and a multi-source training scheme with mixed natural and synthetic data, Lumina-Video achieves remarkable aesthetic quality and motion smoothness at high training and inference efficiency. We additionally propose Lumina-V2A, a video-to-audio model based on Next-DiT, to create synchronized sounds for generated videos. Codes are released at https://www.github.com/Alpha-VLLM/Lumina-Video.

==> table/vbench.tex <==
\begin{table*}[t]
    \caption{Quantitative evaluation results on VBench.}
    \label{tab:vbench}
    \vskip 0.15in
    \begin{center}
        \begin{small}
            \begin{sc}
                \begin{tabular}{ll*{7}{c}*{9}{c}}
                    \toprule
                     &Param& \multicolumn{7}{c}{Quality Score} & \multicolumn{9}{c}{Semantic Score} \\
                    \cmidrule(lr){3-9} \cmidrule(lr){10-18}
                               && Q1 & Q2 & Q3 & Q4 & Q5 & Q6 & Q7 & S1 & S2 & S3 & S4 & S5 & S6 & S7 & S8 & S9 \\
                    \midrule
                    \textit{\textcolor{gray}{proprietary models}} &&&&&&&&&&&&&&&&& \\

                    Gen-3 (2024-07) & - &&&&&&&&&&&&&&&& \\
                    Luma & - &97.33\% &97.43\% &98.64\% &99.35\% &44.26\% &65.51\% &66.55\% &94.95\% &82.63\% &96.40\% &92.33\% &83.67\% &58.98\% &24.66\% &26.29\% &28.13\% \\
                    Kling (2024-07 high-performance) & - &&&&&&&&&&&&&&&& \\
                    Vidu & - &&&&&&&&&&&&&&&& \\
                    Pika-1.0 (2024-06) & - &&&&&&&&&&&&&&&& \\
                    
                    \midrule
                    \textit{\textcolor{gray}{open-source models}} &&&&&&&&&&&&&&&&& \\
                    Allegro & 3B &&&&&&&&&&&&&&&& \\ %2.8B DiT + 175M VAE
                    HunyuanVideo & 13B &&&&&&&&&&&&&&&& \\
                    CogVideoX1.5 & 5B &&&&&&&&&&&&&&&& \\
                    OpenSora V1.2 (8s) & 1.1B &&&&&&&&&&&&&&& \\
                    OpenSoraPlan V1.3 &&&&&&&&&&&&&&&& \\
                    VideoCrafter-2.0 &&&&&&&&&&&&&&&& \\
                    Vchitect-2.0 & 2B &&&&&&&&&&&&&&& \\
                    Pyramid Flow &&&&&&&&&&&&&&&&& \\
                    Lumina-Video-ss &&&&&&&&&&&&&&&&& \\
                    Lumina-Video-ms &&&&&&&&&&&&&&&&& \\
                    \bottomrule
                \end{tabular}
            \end{sc}
        \end{small}
    \end{center}
    \vskip -0.1in
\end{table*}
